Clustering in graphs and hypergraphs with categorical edge labels

Modern graph or network datasets often contain rich structure that goes beyond simple pairwise connections between nodes. This calls for complex representations that can capture, for instance, edges of different types as well as so-called "higher-order interactions" that involve more than two nodes at a time. However, we have fewer rigorous methods that can provide insight from such representations. Here, we develop a computational framework for the problem of clustering hypergraphs with categorical edge labels --- or different interaction types --- where clusters corresponds to groups of nodes that frequently participate in the same type of interaction. Our methodology is based on a combinatorial objective function that is related to correlation clustering on graphs but enables the design of much more efficient algorithms that also seamlessly generalize to hypergraphs. When there are only two label types, our objective can be optimized in polynomial time, using an algorithm based on minimum cuts. Minimizing our objective becomes NP-hard with more than two label types, but we develop fast approximation algorithms based on linear programming relaxations that have theoretical cluster quality guarantees. We demonstrate the efficacy of our algorithms and the scope of the model through problems in edge-label community detection, clustering with temporal data, and exploratory data analysis.

==> experiments-full.tex <==
%!TEX root = main.tex

\begin{table*}[t!]
	\caption{Summary statistics of datasets --- number of nodes $\lvert V \rvert$, number of (hyper)edges $\lvert E \rvert$, 
	maximum hyperedge size $r$, and number of categories $k$ --- along with \obj{}
	performance for the algorithms \emph{LP-round} (LP), \emph{Majority Vote} (MV), \emph{Cat-IsoCut} (IC), 
	\emph{ChromaticBalls} (CB) and \emph{LazyChromaticBalls} (LCB). 
	Performance is listed in terms of the approximation guarantee given by the LP lower bound (lower is better)
	and in terms of the edge satisfaction, which is the fraction of edges that are \emph{not mistakes}
	(higher is better; see \cref{eq:chromec}).
	Our LP method performs the best overall and can even find exactly (or nearly) optimal solutions
	to the NP-hard objective by matching the lower bound.
	We also report the running times for rough comparison, though our implementations are not optimized for efficiency. Due to its simplicity, MV is extremely fast.
	}
	\label{tab:allexp1}
	\centering
	\scalebox{0.95}{\begin{tabular}{l     l l l l     l l l l l     l l l l l    l l l ll}
		\toprule
		&&&&& \multicolumn{5}{c}{\textbf{Approx. Guarantee}} & \multicolumn{5}{c}{\textbf{Edge Satisfaction}} & \multicolumn{5}{c}{\textbf{Runtime (in seconds)}} \\ 
		\cmidrule(lr){6-10} \cmidrule(lr){11-15}  \cmidrule(lr){16-20}
		%\!\!\!\!\!\!\!
		\emph{Dataset} & $\lvert V \rvert$ & $\lvert E \rvert$ & $r$ & $k$ & LP  & MV   & IC   & CB   & LCB  & LP   & MV   & IC   & CB   & LCB  & LP & MV& IC & CB & LCB \\
		\midrule
Brain & 638 & 21180 & 2 & 2 &1.0 & 1.01 & 1.27 & 1.56 & 1.41 & 0.64 & 0.64 & 0.55 & 0.44 & 0.5 & 1.8 & 0.0 & 1.9 & 0.4 & 0.8\\
MAG-10 & 80198 & 51889 & 25 & 10 &1.0 & 1.18 & 1.37 & 1.44 & 1.35 & 0.62 & 0.55 & 0.48 & 0.45 & 0.49 & 51 & 0.1 & 203 & 333 & 699\\
Cooking & 6714 & 39774 & 65 & 20 &1.0 & 1.21 & 1.21 & 1.23 & 1.24 & 0.2 & 0.03 & 0.03 & 0.01 & 0.01 & 72 & 0.0 & 1223 & 4.6 & 6.7\\
DAWN & 2109 & 87104 & 22 & 10 &1.0 & 1.09 & 1.0 & 1.31 & 1.15 & 0.53 & 0.48 & 0.53 & 0.38 & 0.46 & 13 & 0.0 & 190 & 0.3 & 0.4\\
Walmart-Trips & 88837 & 65898 & 25 & 44 & 1.0 & 1.2 & 1.19 & 1.26 & 1.26 & 0.24 & 0.09 & 0.09 & 0.04 & 0.05 & 7686 & 0.2& 68801 & 493 & 1503\\
		\bottomrule
	\end{tabular}}
\end{table*} 

\section{Experiments}\label{sec:experiments}
We now run four types of numerical experiments to test our algorithms and
demonstrate our methodology. First, we show that our algorithms indeed work well
on a broad range of datasets at optimizing our objective function and discover
that our LP relaxation tends be extremely effective in practice, often finding an
optimal solution (i.e., matching the lower bound). After, we show that our
approach is superior to competing baselines in categorical community detection
experiments where edges are colored to signal same-community membership, using
an array of synthetic and real-world data. Next, we show how to use timestamped
edge information as a categorical edge label, and demonstrate that our method
can find clusters that preserve temporal information better than methods that
only look at graph topology, without sacrificing performance on topological
metrics. Finally, we present a case study on a network of cooking ingredients
and recipes to show that our methods can also be used for exploratory data
analysis. Our code and datasets are available at~\url{https://github.com/nveldt/CategoricalEdgeClustering}.

\subsection{Analysis on Real Graphs and Hypergraphs}
\label{sec:exp1}
We begin by evaluating our methods on several real-world edge-labeled graphs and
hypergraphs in terms of \obj{}. The purpose of these experiments is to show
that our methods can optimize the objective quickly and accurately, to compare
our different algorithms for the objective in terms of accuracy and running
time, and to demonstrate that our methods find global categorical clustering
structure better than a natural baseline algorithm. All experiments are run on a
laptop with a 2.2 GHz Intel Core i7 processor and 8 GB of RAM.
We implemented our algorithms in Julia, using Gurobi software to solve the linear programs.
We will release our code and data upon publication.

\xhdr{Datasets}
%We consider five datasets with categorical hyperedge labels.
\Cref{tab:allexp1} provides summary statistics of the datasets we use, and
we briefly describe them below.
%
\emph{Brain}~\cite{crossley2013cognitive} is a graph where nodes represent brain regions from an MRI.
There are two edge categories: one for connecting regions with high fMRI correlation
and one for connecting regions with similar activation patterns.
%
In the Drug Abuse Warning Network (\emph{DAWN})~\cite{DAWN-data},
nodes are drugs, hyperedges are
combinations of drugs taken by a patient prior to an emergency room visit, and
edge categories indicate the patient disposition (e.g., ``sent home'', ``surgery'',
``released to detox'').
%
The \emph{MAG-10} network is a subset of the Microsoft Academic
Graph~\cite{MAG-data} where nodes are authors, hyperedges correspond to a
publication from those authors, and there are 10 edge categories which denote
the computer science conference publication venue (e.g., ``WWW'', ``KDD'',
``ICML''). If the same set of authors published at more than one conference, we
used the most common venue as the category, discarding any cases where there is
a tie.
%
In the \emph{Cooking} dataset~\cite{cooking-data},
nodes are food ingredients, hyperedges are
recipes made from combining multiple ingredients, and categories indicate cuisine
(e.g., ``Southern-US'', ``Indian'', ``Spanish'').
%
Finally, the \emph{Walmart-Trips} dataset is made up of products (nodes), groups of
products purchased during a single grocery run (hyperedges), and categories are
44 unique ``trip types'', as classified by Walmart~\cite{walmart-data}.

%Should the manuscript be accepted, we will provide a link for accessing all datasets and code.

\xhdr{Algorithms}
We use two algorithms that we developed in
\cref{sec:morecats}. The first is the simple 2-approximation rounding scheme
outlined in \cref{alg:2round}, which we refer to as \emph{LP-round} (\emph{LP}) (in
practice, this performs as well as the more sophisticated algorithm in
\cref{alg:rand} and has the added benefit of being deterministic).  The second
is \emph{Cat-IsoCut} (\emph{IC}), which runs the standard isolating cut
heuristic~\cite{Dahlhaus94thecomplexity} on an instance of multiway cut derived
from the \obj{} problem, as outlined in \cref{sec:mwc}.

The first baseline we compare against is \emph{Majority Vote} (\emph{MV}), 
which assigns node $i$ to category $c$ if $c$ is the most
common edge type in which $i$ participates. The result of \emph{MV} is also
used as the default cluster assignment for \emph{IC}, since in practice
this method may leave some nodes unattached from all terminal nodes.

The other baselines are \emph{Chromatic Balls} (\emph{CB}) and \emph{Lazy
  Chromatic Balls} (\emph{LCB}) --- two algorithms for chromatic
correlation clustering~\cite{Bonchi2015ccc}. These methods repeatedly select
an unclustered edge, and greedily grow a cluster around it by adding nodes
that share edges with the same label. Unlike our methods, \emph{CB} and
\emph{LCB} distinguish between category (color) assignment and cluster
assignment: two nodes may be colored the same but placed in different
clusters. To provide a uniform comparison among methods, we merge distinct
clusters of the same category into one larger cluster.  These methods are
\emph{not} designed for hypergraph clustering, but we still use them for
comparison by reducing a hypergraph to an edge-labeled graph, where nodes
$i$ and $j$ share an edge in category $c$ if they appear together in more
hyperedges of category $c$ than any other.

\xhdr{Results}
Table~\ref{tab:allexp1} reports how well each algorithm solves the \obj{} objective. We report both the approximation guarantee (the ratio between each algorithm's output and the LP lower bound), as well as the \emph{edge satisfaction}, which measures the fraction of hyperedges that end up inside a cluster with the correct label. Observe that maximizing edge satisfaction is equivalent to minimizing the number of edge label mistakes. 
%Reporting edge satisfaction provides an intuitive way to interpret and analyze our results. 
%High edge satisfaction scores imply that a dataset is indeed characterized by large groups of objects that tend to interact in a certain way with other members of the same group. A very low satisfaction score for a dataset indicates that assigning a single label to each node may be insufficient to capture the intricacies of the dataset. Thus, further exploration and pre-processing of the data may be necessary. We explore this in depth in Section~\ref{sec:exp3}.
In all cases, the LP solution is integral or nearly integral, indicating that \emph{LP} does an extremely good job solving the original NP-hard objective, often finding an exactly-optimal solution. 
As a result, it outperforms all other methods on all datasets. Furthermore, on nearly all datasets, we can solve the LP within a few seconds or a few minutes. \emph{Walmart} is an exception--given the large number of hyperedge labels, the LP contains nearly 4 million variables, and far more constraints. The baseline algorithms \emph{MV}, \emph{LCB}, and \emph{CB} are typically faster, 
but they do not perform as well in solving the objective. 

The high edge satisfaction scores indicate that our method does the best job identifying sets of nodes which \emph{as a group} tend to participate in one specific type of interaction. In contrast, the \emph{MV} algorithm identifies nodes that {individually} exhibit a certain behavior, but the method does not necessarily form clusters of nodes that as a group interact in a similar way. Because our \emph{LP} method outperforms our \emph{IC} approach 
on all datasets in terms of both speed and accuracy, in the remaining experiments we focus only on comparing \emph{LP} against other competing algorithms.

\subsection{Categorical Edge Community Detection}
Next we demonstrate the superiority of \emph{LP} in detecting communities of nodes with the same node labels (i.e., \emph{categorical communities}), based on labeled edges between nodes. We perform experiments on synthetic edge-labeled graphs, as well as two real-world datasets, where we reveal edge labels indicative of the ground truth node labels and see how well we can recover the node labels.

\xhdr{Synthetic Model}
We use the synthetic random graph model designed by Bonchi et al.\ for chromatic correlation clustering~\cite{Bonchi2015ccc}. For this model, a user specifies the number of nodes $n$, colors $L$, and clusters $K$, as well as edge parameters $p$, $q$, and $w$. The model first assigns nodes to clusters uniformly at random, and then assigns clusters to colors uniformly at random. \textcolor{blue}{Due to this random assignment procedure, some of the cluster numbers and colors may not be used. Thus, $K$ and $L$ are in fact upper bounds on the number of distinct clusters and unique colors used.}
For nodes $i$ and $j$ in the same cluster, the model connects them with an edge with probability $p$. 
With probability $1-w$, the edge is given the same color as $i$ and $j$. Otherwise, it is given a uniform random color. 
If $i$ and $j$ are in different clusters, an edge is drawn with probability $q$, and given a uniform random color. 
We will also use a generalization of this model to synthetic $r$-uniform hypergraphs. The difference is that we assign colored hyperedges to $r$-tuples of the $n$ nodes, rather than just pairs, and we assign each cluster to a unique color. %Again, in our problem, colors and categories are the same.


\xhdr{Synthetic Graph Results}
We set up three experiments, where performance is measured by the fraction of nodes
placed in the correct cluster (node label accuracy).
In the first, we form graphs with $n = 1000$, $p = 0.05$, and $q = 0.01$, fixing $L = K = 15$, \textcolor{blue}{which in practice leads to graphs with 15 clusters and typically between 8 and 12 distinct edge and cluster colors.} 
We then vary the noise parameter $w$ from $0$ to $0.75$ in increments of $0.05$. 
\Cref{fig:noise} reports the median accuracy over 5 trials of each method for each value of $w$.
In the second, we fix the noise level $w = 0.2$, and vary the number of clusters $K$ from 5 to 50 in increments of 5
with $L = K$.
\Cref{fig:clusters} reports the median accuracy over 5 trials for each value of $K$.
In both experiments, our LP-round method substantially outperforms the others,
although the methods perform more similarly for high noise levels or large numbers of clusters. \textcolor{blue}{For our first two experiments, we additionally found that our LP algorithm similarly outperformed other methods in terms of cluster identification scores such as Adjusted Rand Index and F-score, followed in performance by MV. Cluster identification scores for LCB and CB were particularly low (ARI scores always below 0.02), as these methods tended to form far too many clusters.} 

%We additionally checked \emph{cluster} identification scores such as Adjusted Rand Index (ARI), and F-scores. Our LP algorithm continues to outperform other methods in terms of these scores, followed by MV. LCB and CB obtain particularly low ARI and F-scores, as they tend to form too many clusters.
\begin{figure}[t]
	\centering
	\subfloat[Graphs: Varying Noise $w$ \label{fig:noise}]
	{\includegraphics[width=.475\linewidth]{Figures/Vary_w_graph}}\hfill
	\subfloat[Graphs: Varying \# Clusters \label{fig:clusters}]
	{\includegraphics[width=.475\linewidth]{Figures/VaryKL_graph}}\hfill
	\subfloat[Hypergraphs: Varying Noise $w$ \label{fig:noise-hyper}]
	{\includegraphics[width=.475\linewidth]{Figures/Hypergraph_vary_w}}\hfill
	\subfloat[Hypergraphs: Varying \# Clusters \label{fig:clusters-hyper}]
	{\includegraphics[width=.475\linewidth]{Figures/Hypergraph_vary_kl}}
	\caption{(a)--(b): Performance of algorithms on a synthetic graph model for chromatic correlation clustering~\cite{Bonchi2015ccc}. Across a range of parameters, \emph{LP-round} outperforms competing methods in predicting the ground truth label of the nodes. (c)--(d) In experiments on synthetic 3-uniform hypergraphs, \emph{LP-round} performs well for most parameter regimes but there is some sensitivity to the very noisy setting.}
	\label{fig:synthetic_all}
\end{figure}

\textcolor{blue}{The CB and LCB algorithms, as well as the synthetic graph model itself, explicitly distinguish between ground truth node labels and ground truth clusters. Thus, our third experiment explores a parameter regime tailored more towards the strengths of CB and LCB. We fix $L = 20$, and vary the number of clusters from $K = 50$ to $K = 200$ in increments of 25. Following the experiments of Bonchi et al.~\cite{Bonchi2015ccc} we set $p = w = 0.5$, and set $q = 0.03$. Even in this setting, we find that our algorithms maintain an advantage. For all values of $K$, our LP algorithm outperforms other methods in terms of node label accuracy, and also obtains higher ARI scores when $K$ is a small multiple of $L$. We note that LCB and CB only obtain better cluster identification scores in parameter regimes where all algorithms obtain ARI scores below 0.1.}
%This is not surprising, given the node accuracy results in \Cref{acc}. When the number of clusters is large, all methods have low node labeling accuracy. Since all nodes in the same cluster have the same node label, we do not expect any method to accurately identify clusters if they are unable to identify node labels.
\begin{figure}[t]
	\centering
	\subfloat[Label Accuracy \label{acc}]
	{\includegraphics[width=.475\linewidth]{Figures/Graph_Large_K_Accuracy}}\hfill
	\subfloat[ARI Scores \label{ari}]
	{\includegraphics[width=.475\linewidth]{Figures/Graph_Large_K_ARI}}
	\caption{ \textcolor{blue}{LCB and CB are primarily designed for settings where $K$ is much larger than $L$. Despite this, our LP method always obtains better label assignment scores, and often obtains better ARI cluster identification scores, when we fix $L = 20$ and let $K$ vary from 50 to 500.}}
	\label{fig:bonchiexps}
%	\vspace{-.5\baselineskip}
\end{figure}

\xhdr{Synthetic Hypergraph Results}
We run similar experiments on synthetic 3-uniform hypergraphs. 
%For hypergraphs, we deviate slightly from the synthetic graph model of Bonchi et al.~\cite{Bonchi2015ccc} in that we assign each cluster to its own unique label, rather than letting different ground truth clusters share the same label. 
We again set $n = 1000$, and use $p = 0.005$ and $q = 0.0001$ for in-cluster and between-cluster hyperedge probabilities. In one experiment we fix $L = 15$ and vary $w$, and in another we fix $w = 0.2$ and vary number of clusters $L$. \Cref{fig:noise-hyper,fig:clusters-hyper} display node labeling accuracy results. Again, we see that \emph{LP} tends to have the best performance. When $L = 15$ and we vary $w$, our method achieves
nearly perfect accuracy for $w \le 0.6$.
However, we observe performance sensitivity when the noise becomes large enough:
when $w$ increases from $0.6$ to $0.65$, the output of \emph{LP} no longer tracks the ground truth cluster assignment. This occurs despite the fact that the LP solution is integral, and we are in fact optimally solving the \obj{} objective. Therefore, we conjecture this sharp change in node label accuracy is due to an information theoretic detectability threshold, which depends on parameters of the synthetic model.
%\begin{figure}[t]
%	\centering
%	\subfloat[Varying Noise $w$ \label{fig:noise-hyper}]
%	{\includegraphics[width=.475\linewidth]{Figures/Hypergraph_vary_w}}\hfill
%	\subfloat[Varying \# of Clusters \label{fig:clusters-hyper}]
%	{\includegraphics[width=.475\linewidth]{Figures/Hypergraph_vary_kl}}
%	\caption{In synthetic 3-uniform hypergraphs, algorithmic performance is very sensitive to changes in the model parameters. For many parameter regimes, however, \emph{LP-round} obtain near perfect accuracy.}
%	\label{fig:synthetic3}
%\end{figure}

%\begin{figure}[t]
%	\centering
%	\includegraphics[width=.65\linewidth]{Figures/Vary_w_hypergraph}
%		\vspace{-.5\baselineskip}
%	\caption{
%		In synthetic 3-uniform hypergraphs, algorithmic performance is very sensitive to changes in the model parameters. For many parameter regimes, however, \emph{LP-round} obtain near perfect accuracy.}
%	\label{fig:synthetic3}
%\end{figure}


\xhdr{Academic Department Labels in an Email Network} 
To test the algorithms on real-world data, we use the \emph{Email-Eu-core} network~\cite{yin2017local,leskovec2007graph}.
Nodes in the graph represent researchers at a European institution, 
edges indicate email correspondence (we consider the edges as undirected), 
and nodes are labeled by the departmental affiliation of each researcher. 
We wish to test how well each method can identify node labels, 
if we assume we have access to a (perhaps noisy and imperfect) mechanism for associating emails with labels for inter- and intra-department communication. 
To model such a mechanism, we generate edge categories in a manner similar to a model from Bonchi et al.~\cite{Bonchi2015ccc}. 
An edge inside of a cluster (i.e., an email within the same department) is given the correct department label with probability $1-w$, and a random label with probability $w$. 
An edge between two members of different departments is given a uniform random label. 
\Cref{fig:email2} reports each algorithm's ability to detect department labels when $w$ varies from $0$ to $0.75$. Our LP-round
method returns the best results in all cases, and is robust in detecting department labels even in the high-noise regime.
\begin{figure}[t]
	\centering
	\subfloat[Email-Eu-core \label{fig:email2}]
	{\includegraphics[width=.5\linewidth]{Figures/Email-Departments-Accuracy}}\hfill
	\subfloat[Walmart-Products \label{fig:walmart}]
	{\includegraphics[width=.5\linewidth]{Figures/Walmart-Product-Accuracy}}\hfill
	\caption{
	Accuracy in clustering nodes in real-world datasets when edge labels are made to be a 
	noisy signal for ground truth membership.
	For both an email graph (a) and a product co-purchasing hypergraph (b), our \emph{LP-round} method
	consistently outperforms other methods in inferring ground truth node labels from edge labels.
	}
	\label{fig:real-cd}
\end{figure}

\xhdr{Walmart Product Categories}
The \emph{Walmart-Trips} dataset from \cref{sec:exp1} also has product information.
We assigned products to one of ten broad departments in which the product appears on \url{walmart.com}
(e.g., ``Clothing, Shoes, and Accessories'') to construct a \emph{Walmart-Products} hypergraph 
with ground truth node labels (we will release this dataset with the paper).
Recall that hyperedges are sets of co-purchased products. 
We generate noisy hyperedge labels as before, with $1-w$ defining the probability that a hyperedge with nodes from a single department label will have the correct label. 
Results are reported in \cref{fig:walmart}, and our
LP-round method can detect true departments at a much higher rate than the other methods.

\subsection{Temporal Community Detection}
In the next experiment, we show how our framework can be used to identify
communities of nodes in a temporal network, where we use timestamps on edges as
a type of categorical label that two nodes should be clustered together. For
data, we use the \emph{CollegeMsg} network~\cite{panzarasa2009patterns}, which
records private messages (time-stamped edges) between 1899 users (nodes) of a
social media platform at UC Irvine.

Removing timestamps and applying a standard graph clustering algorithm would be
a standard approach to identify communities of users that share a large number
of interactions with each other. However, this loses the explicit relationship
with time. As an alternative, we convert time stamps into discrete edge labels
by ordering edges with respect to time and separating them into $k$ equal sized
bins, representing time windows. Optimizing \obj{} then corresponds to
clustering users into time windows, in order to maximize the number of private
messages that occur between users in the same time window. In this way, our
framework can identify \emph{temporal communities} in a social network, i.e.,
groups of users that are highly active in sending each other messages
\emph{within a short period of time}.
\begin{figure}[t]
	\centering
	\subfloat[Normalized Cut \label{fig:normcut}]
	{\includegraphics[width=.475\linewidth]{Figures/Normcuts}}\hfill
	\subfloat[Inner edge time difference \label{fig:avgtimediff}]
	{\includegraphics[width=.475\linewidth]{Figures/Timedev}}
	\caption{Results for \emph{LP-round} and \emph{Graclus} in clustering a temporal network.
          Our \emph{LP-round} method is competitive for \emph{Graclus}'s objective (normalized cut; left),
          while preserving the temporal structure of network much better (right).}
	\label{fig:temporal}
\end{figure}

We construct edge-labeled graphs for different values of $k$, and run
\emph{LP-round} on each graph. We compare this against clusterings obtained by discarding time stamps and running \emph{Graclus}~\cite{Dhillon-2007-graclus},
a standard graph clustering algorithm, to form $k$ clusters.
\emph{Graclus} seeks to cluster the nodes into $k$ disjoint clusters
$S_1, \ldots, S_k$ to minimize the normalized cut objective:
\begin{equation*}
\label{normcut}
{\textstyle \textbf{Ncut}(S_1, S_2, \hdots, S_k) =\sum_{i = 1}^k \frac{\textbf{cut}(S_i)}{\textbf{vol}(S_i)}},
\end{equation*}
where $\textbf{cut}(S)$ is the number of edges leaving $S$, and
$\textbf{vol}(S)$ is the \emph{volume} of $S$, i.e., the number of edge end
points in $S$. \Cref{fig:normcut} shows that \emph{LP-round} is in fact
competitive with \emph{Graclus} in finding clusterings with small normalized cut
scores, even though \emph{LP-round} is designed for a different objective.
However, \emph{LP-round} still tries to avoid cutting edges, and it happens to find clusterings that also have small normalized cut values. The other goal of \emph{LP-round} is to place few edges in a cluster
with the wrong label, which in this scenario corresponds to clustering private
messages together if they happen close to each other in time. We therefore also
measure the average difference between timestamps of interior edges and the
average time stamp in each clustering, i.e.,
\begin{equation*}
\label{timediff}
{\textbf{AvgTimeDiff}(S_1, \hdots, S_k) = \frac{1}{\lvert E_{\textnormal{int}} \rvert}\sum_{i = 1}^k \sum_{e\in E_i} \lvert \text{timestamp}(e) - \mu_i \rvert, }
\end{equation*}
where $E_{\textnormal{int}}$ is the set of interior edges completely contained
in some cluster, $E_i$ is the set of interior edges of cluster $S_i$, and
$\mu_i$ is the average time stamp in $E_i$. Not surprisingly, this value tends
to be large for \emph{Graclus}, since this method ignores time stamps and only
seeks clusters of highly active users. However, \Cref{fig:avgtimediff}
shows that this value tends to be small for \emph{LP-round}, indicting that it
is indeed detecting clusters of users that are highly interactive within a
specific short period of time.

\subsection{Analysis of the Cooking Hypergraph}
\label{sec:exp3}
Finally, we apply our framework and LP-round algorithm to gain insights into the
\emph{Cooking} hypergraph dataset used in \cref{sec:exp1} and to demonstrate the
capabilities of our methodology for exploratory data analysis. Recall that an
edge in this hypergraph is a set of ingredients for a recipe, and that this
recipe is categorized according to cuisine. Optimizing the \obj{} objective
thus corresponds to separating ingredients among cuisines, in a way that
maximizes the number of recipes whose ingredients are all in the same cluster
(see Ahn et al.~\cite{Ahn-2011-flavor} for related analyses).

\xhdr{Removing high-degree ingredients}
\Cref{tab:allexp1} shows that only 20\% of the recipes can
be made (i.e., a 0.2 edge satisfaction) after partitioning ingredients among
cuisine types.  This is due to the large number of common ingredients such as
salt and olive oil that are shared across many cuisines (a problem noted in
other network analyses of recipes~\cite{Teng-2012-recipes}). We wish to remove
the negative effect of these high-degree nodes.  For an ingredient $i$, let
$d_i^c$ be the number of recipes of cuisine $c$ containing $i$. Let
$M_i = \max_{c} d_i^c$ measure \emph{majority degree} and $T_i = \sum_{t} d_i^c$ the
\emph{total degree}.  Note that $B_i = T_i - M_i$ is a lower bound on the number
of hyperedge mistakes we will make at edges incident to node $i$. We can refine
the original dataset by removing all nodes with $B_i$ greater than some $\beta$.

\xhdr{Making recipes or wasting ingredients}
\begin{figure}[t]
	\centering
	\subfloat[Edge Satisfaction \label{fig:esat}]
	{\includegraphics[width=.45\linewidth]{Figures/EdgeSat_ingredients}}\hfill
	\subfloat[Unused ingredients \label{fig:unused}]
	{\includegraphics[width=.475\linewidth]{Figures/Unused_ingredients}}\hfill
	\caption{As $\beta$ increases, we discard fewer high-degree ingredients before clustering the rest. Our method
	 always ``makes'' more recipes (higher edge satisfaction) and ``wastes'' fewer ingredients (smaller \# of unused ingredients).}
	\label{fig:cooking}
\end{figure}
Figure~\ref{fig:esat} shows edge satisfaction scores for \emph{LP} and
\emph{MV} when we cluster the dataset for different parameters $\beta$. When
$\beta = 10$, we achieve an edge satisfaction above 0.64 with \emph{LP}. As
$\beta$ increases, edge satisfaction decreases, but \emph{LP} outperforms
\emph{MV} in all cases. We also consider a measure of ``ingredient
waste'' for each method. An ingredient is \emph{unused} if we cannot make any
recipes by combining the ingredient with other ingredients in its cluster. A low
number of unused ingredients indicates that a method forms clusters where
ingredients tend to combine together well. \Cref{fig:unused} shows the number of
unused ingredients as $\beta$ varies. Again, \emph{LP} outperforms \emph{MV}.

\xhdr{Specific ingredient and recipe clusters} 
\begin{table}[t]
	\caption{Examples of ingredients and recipes from special clusters identified by \emph{LP-round}, but not \emph{Majority Vote}.}
	\label{tab:clusters}
	\centering
	\begin{tabular}{p{\linewidth}}
		\toprule
		\textbf{French Fruit-Based Desserts} ($\beta = 70$)\\ 
		\textbf{Ingredients:} ruby red grapefruit, strawberry ice cream, dry hard cider, icing, prunes, tangerine juice, sour cherries.\\
		 \textbf{Recipes:} 1. \{almond extract, bittersweet chocolate, sugar, sour cherries, brioche, heavy cream, unsalted butter, kirsch\}, 2. \{large egg yolks, ruby red grapefruit, dessert wine, sugar\}\\
		\midrule 
		\textbf{Brazilian Caipirinha Recipes} ($\beta = 170$) \\
		\textbf{Ingredients:} simple syrup, light rum, ice, superfine sugar, key lime, coco, kumquats, liquor, mango nectar, vanilla essence\\
		 \textbf{Recipes:} \{cachaca, ice\} $+$ 
		1. \{ lime juice, kumquats, sugar\},
		2. \{lime, fruit puree, simple syrup\},
		3. \{ superfine sugar, lime juice, passion fruit juice\},
		4. \{ sugar, liquor, mango nectar, lime, mango\}\\
		\bottomrule
	\end{tabular}
\end{table} 
We finally highlight specific ingredient clusters that \emph{LP} identifies but \emph{MV} does not. When $\beta = 170$, \emph{LP} places 10 ingredients with the Brazilian cuisine which \emph{MV} does not, leading to 23 extra recipes that are unique to \emph{LP}. Of these, 21 correspond to variants of the Caipirinha, a popular Brazilian cocktail. When $\beta = 70$, 24 ingredients and 24 recipes are unique to the French cuisine cluster of \emph{LP}. Of these, 18 correspond to desserts, and 14 have a significant fruit component. 
%Many also correspond to dessert drink cocktails and involve fruit brandy (e.g., calvados, armagnac, eau de vie). 
Table~\ref{tab:clusters} displays examples of ingredients and recipes in from both these clusters.
%We note also that \emph{LP} identifies ingredients and recipes for an Irish cake and dessert cluster, and a British cuisine cluster with several savory beef dishes and pie recipes.

